Modeling the Saturation of the Bell Instability using Hybrid Simulations

The nonresonant streaming instability (Bell instability) plays a pivotal role in the acceleration and confinement of cosmic rays (CRs); yet, the exact mechanism responsible for its saturation and the magnitude of the final amplified magnetic field have not been assessed from first-principles. Using a survey of hybrid simulations (with kinetic ions and fluid electrons), we study the evolution of the Bell instability as a function of the parameters of the CR population. We find that, at saturation, the magnetic pressure in the amplified field is comparable with the initial CR anisotropic pressure, rather than with the CR energy flux as previously argued. These results provide a predictive prescription for the total magnetic field amplification expected in the many astrophysical environments where the Bell instability is important.

==> scratch.tex <==


$$\xi_0 = \frac{T^{11}-p}{P_{B,0}} = \frac{T^{00}-\tilde{\rho}c^2}{P_{B,0}} = \frac{T^{01}}{P_{B,0}} \frac{v_{bst}}{c} \; .$$







We note that \ref{eq:xibellcold} has the same non-relativistic and relativistic limits of 
\begin{equation}
    \xi = \eta (\gamma_d-1)\frac{c^2}{v_A^2}=T^{00}-\rho_{cr}c^2,
\end{equation}
which expresses the density of kinetic energy.

Let's then try the generic expression for finite $p_{iso}$, which reads
\begin{equation}
    T^{00}=\gamma_d^2 (e+p)-p,
\end{equation}
where $e= \gamma_{iso} \tilde{\rho}_{cr}c^2$ and 
$p=\frac13 \gamma_{iso}\tilde{\rho}_{cr}c^2\beta_{iso}^2$.
Eventually, after some easy algebra:
\begin{equation}\label{eq:xinew}
    \xi= 2\gamma\I\frac{n\C}{n_g} \frac{c^2}{v_A^2}\left(\gamma_d-1+\frac{\gamma_d}{3}\beta_d^2\beta\I^2\right).
\end{equation}
\begin{equation}\label{eq:xinew2}
    \xi= 2\gamma\I\frac{n\C}{n_g} \frac{c^2}{v_A^2}\left(\gamma_d-1+\frac{\gamma_d}{3}\frac{v_d^2}{c^2}\frac{v\I^2}{c^2}\right).
\end{equation}
In the Bell limit (relativistically hot, non-rel drift), this reduces to:
\begin{equation}
    \xi= \gamma_{iso}\eta \frac{v_d^2}{v_A^2}.
\end{equation}
Compared to Bell's prescription:
\begin{equation}
    \frac{\xi}{\xi_B}= \frac{2v_d}{c},
\end{equation}
so, we always saturate at lower value than predicted by Bell.

On the other hand, what if the boost is relativistic?
Bell's argument is that at saturation $k_{max}r_L\sim 1$, so for a ultra-rel beam with $p_d\gg p\I$ one should calculate $r_L$ with $p_d=\gamma_d m v_d$ rather than with $p_\perp$, so 
\begin{equation}
    \xi_B = \eta \gamma_{d}\frac{c^2}{v_A^2}, 
\end{equation}
which is equivalent to Eq. \ref{eq:xinew}, modulo a factor of 2 that may come from the improper treatment of the relativistic term. 
In this limit $U_{cr}\sim\gamma_d m c^2$, so essentially $\xi$ is still the one in Eq. \ref{eq:xibell} with $v_d\sim c$.

In summary, we are concluding that Bell's estimate is too optimistic for non-rel drifts, but should still apply to the beam of the escaping particles if they are relativistic. 
Another way of saying this is that Bell's estimate relies also on transforming the rest mass energy into B, which is unphysical. 








In order to describe the energy/momentum in the CR distribution, it is useful to introduce the CR stress-energy tensor \citep[see, e.g., \S133  of][]{landau6} $T\C^{\mu\nu}$ (with $\mu,\nu=0,1,2,3$), where  $T^{01}\C/c$ and $cT^{01}\C$ are the CR density of momentum {\bf along $i $} and the energy flux along $x$, respectively. 
Defining also $\gamma\D $ as the Lorentz factor associated  with the CR drift $v\D $, we generally have
\begin{equation}
    T^{01}\C= \left( \gamma\I \tilde{n}\C m c^2+\frac{1}{3} \tilde{n}\C p\I v\I \right) \gamma\D ^2 \frac{v\D }{c},
\end{equation}
where the first term in the parenthesis is the CR energy density (mass+internal) and the second is the pressure in the CR rest frame;
here $\tilde{n}\C={n}\C/\gamma\D $ 
is the CR density in their reference frame, which is \emph{smaller} than the one in the simulation frame.
Eventually, we define the quantity
\begin{equation}\label{eq:Pi_cr}
    \Pi\C \equiv T\C^{01}= n\C p\D  c \gamma\I \left( 1 + \frac{1}{3} \frac{v\I^2}{c^2} \right) \;,
\end{equation}
which expresses the net free energy for an arbitrary CR distribution.

Note that $\Pi\C$ has the dimensions of a pressure (i.e. a momentum flux), but it does not include the isotropic pressure associated with $p\I$.
In fact, if $p\I\to 0$ (cold beam) then $\Pi\C \to n\C p\D c$ and $T\C^{01}/c$ is the density of momentum along $x$, while $\Pi\C=0$ for $v\D =0$ (no drift).
Finally, while the term in parentheses is capped at 4/3, the CR momentum flux  $\Pi\C\propto \gamma\I$ scales with how fast the CRs are, even for non-relativistic boosts.

A useful quantity to define is the ratio of $\Pi\C$ to the initial magnetic field pressure, $P_{\rm B,0} = B_0^2/(8\pi)$, i.e.,
\begin{equation}
    \xi\equiv\frac{\Pi\C}{P_{\rm B,0}}=
    \frac{8\pi \gamma\I n\C}{B_0^2} \left( 1+\frac{1}{3}\frac{v\I^2}{c^2}\right) c p\D ,
\end{equation}
which can be conveniently written in terms of the normalized quantities used in the code as:
\begin{equation}\label{eq:xi_new}
    \xi= 2
    \gamma\I \frac{n\C}{n_{\rm g}} \frac{p\D }{mv_{\rm A,0}}
    \frac{c}{v_{\rm A,0}} \left(1+\frac{1}{3}\frac{v\I^2}{c^2}\right).
\end{equation}

The case that is often considered (e.g., in the upstream of non-relativistic shocks) is that of hot drifting CR distribution, for which
\begin{equation}\label{eq:Pi_shock}
    \Pi\C= \frac43 \gamma\I n\C mc v\D  = 4 P\C \frac{v\D }{c}
\end{equation}
and hence 
\begin{equation}\label{eq:xi_shock}
\xi = 4 \frac{P\C}{P_{\rm B,0}}\frac{v\D }{c},
\end{equation}
where $P\C=\frac13 \gamma\I n\C mc^2$ is the CR pressure.
In this case the fastest-growing mode has a wavenumber:
\begin{equation}\label{eq:krho}
k_{\max} r_{\rm L} =  \frac{4\pi}{c}\frac{J\C}{B_0}\frac{pc}{eB_0}
= \frac{3}{2} \frac{P\C}{P_{\rm B,0}} \frac{v\D }{c}= \frac{3}{8} \xi \; ,
\end{equation}
where $r_{\rm L} \equiv pc/(eB_0)$ is the CR Larmor radius.

In its canonical derivation \citep[e.g.,][]{bell04,amato+09}, the Bell instability grows faster than the resonant streaming instability if $k_{\max} r_{\rm L} \gtrsim 1$, i.e., $\xi\gtrsim 2$, and the fastest-growing mode has necessarily a wavelength much smaller than the CR gyroradius (Equation \ref{eq:krho}).
The formalism introduced in this section generalizes such a condition to arbitrary CR distributions.



\subsection{Growth rate and saturation}
While the growth rate and the most unstable modes are fully defined by the CR current, the level of the field amplification at saturation may not depend on it, solely. 
Physically speaking, one would expect the saturation to depend also on the amount of free energy flux in the CR distribution, and hence on $\xi$.
Several possible saturation mechanisms have been proposed in the literature, which can be summarized in two main categories: 
\begin{itemize}
    \item Achievement of energy equipartition between CRs and self-generated magnetic turbulence  \citep[e.g.,][]{bell04,bell05,blasi+15};
    \item Disruption of the CR current due to the scattering of CRs on non-linear waves  and consequent  reduction of the relative drift between CRs and thermal plasma  \citep[e.g.,][]{riquelme+09,ohira+09,gargate+10,caprioli+14b}.
\end{itemize}
Here, we provide the first simulation-based prescription for the level of magnetic field amplification achieved for a given initial CR distribution and discuss how it depends on the available CR energy, parametrized by $\xi$.

